Session Type Inference in Haskell

We present an inference system for a version of the Pi-calculus in Haskell for the session type proposed by Honda et al. The session type is very useful in checking if the communications are well-behaved. The full session type implementation in Haskell was first presented by Pucella and Tov, which is 'semi-automatic' in that the manual operations for the type representation was necessary. We give an automatic type inference for the session type by using a more abstract representation for the session type based on the 'de Bruijn levels'. We show an example of the session type inference for a simple SMTP client.

==> eptcsdata.tex <==
\providecommand{\firstpage}{74}
\providecommand{\publicationstatus}{K. Honda and A. Mycroft (Eds.): Programming Language\\
Approaches to Concurrency and communication-cEntric\\
Software 2010 (PLACES'10)\\
EPTCS 69, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.69.6}{10.4204/EPTCS.69.6}}
\pdfoutput=1

